Signal Propagation in a Gradient-Based and Evolutionary Learning System

Generative adversarial networks (GANs) exhibit training pathologies that can lead to convergence-related degenerative behaviors, whereas spatially-distributed, coevolutionary algorithms (CEAs) for GAN training, e.g. Lipizzaner, are empirically robust to them. The robustness arises from diversity that occurs by training populations of generators and discriminators in each cell of a toroidal grid. Communication, where signals in the form of parameters of the best GAN in a cell propagate in four directions: North, South, West, and East, also plays a role, by communicating adaptations that are both new and fit. We propose Lipi-Ring, a distributed CEA like Lipizzaner, except that it uses a different spatial topology, i.e. a ring. Our central question is whether the different directionality of signal propagation (effectively migration to one or more neighbors on each side of a cell) meets or exceeds the performance quality and training efficiency of Lipizzaner Experimental analysis on different datasets (i.e, MNIST, CelebA, and COVID-19 chest X-ray images) shows that there are no significant differences between the performances of the trained generative models by both methods. However, Lipi-Ring significantly reduces the computational time (14.2%. . . 41.2%). Thus, Lipi-Ring offers an alternative to Lipizzaner when the computational cost of training matters.

==> ack.tex <==
\section*{Acknowledgments}
\label{sec:acks}
This research was partially funded by European Union’s Horizon 2020 research and innovation programme under the Marie Skłodowska-Curie grant agreement No 799078 and by H2020-ICT-2019-3, RTC-2017-6714-5, TIN2017-88213-R, and UMA18-FEDERJA-003 projects. 
The Systems that learn initiative at MIT CSAIL.



==> background-long.tex <==
\section{Related Work}
\label{sec:related-work}
%GAN Training


This section introduces the main concepts in GANs training and
summarizes some studies related with research. 

\vspace{-0.2cm}
\subsection{General GAN training}
\label{sec:gan-training}


GANs train two DNN, a generator ($G_g$) and a discriminator ($D_d$), in an adversarial setup. 
Here, $G_g$ and $D_d$ are functions parametrized by $g$ and $d$, 
where $g \in \calU$ and $d \in \calV$ with $\calU, \calV \subseteq \R^{p}$
represent the respective parameters space of both functions. 

Let $G_*$ be the target unknown distribution to which we would like to fit our generative model~\cite{arora2017generalization}. 
The generator $G_g$ receives a variable from a latent space $z\sim P_{z}(z)$ and creates a sample from data space $x = G_{g}(z)$. 
The discriminator $D_d$ assigns a probability $p = D_{d}(x) \in [0, 1]$ that represents the likelihood that the $x$ belongs to the real training dataset, i.e., $G_*$ by applying a \textit{measuring function} $\phi:[0,1] \to \mathbb{R}$. 
The $P_{z}(z)$ is a prior on $z$ (a uniform $[-1, 1]$ distribution is typically chosen). The goal of GAN training is to find $d$ and $g$ parameters to optimize the objective function $\mathcal{L}(g,d)$.

\begin{equation}
\label{eq:gan-def}
\min_{g\in \mathbb{G}}\max_{d \in \mathbb{D}} \mathcal{L}(g,d),\ \text{where} 
\end{equation}
\begin{equation}
\mathcal{L}(g,d) = \mathbb{E}_{x\sim P_{data}(x)}[\phi (D_d(x))] + \mathbb{E}_{x\sim G_{g}(z)}[\phi(1-D_d(x))] \nonumber
\end{equation}

%In practice, we have access to a finite number of training samples $x_1,
%\ldots, x_m \sim G_*$. Therefore, an empirical version
%$\frac{1}{m}\sum_{i=1}^{m} \phi(D_d(x_i))$ is used to estimate
%$\E_{x\sim G_*}[\phi (D_d(x))]$. The same also holds for $G_g$.

Thus, during the learning process $D_d$ learns a binary classifier providing the best possible discrimination between real and fake
data.
Simultaneously, it encourages $G_g$ to fit the real data
distribution. In general, both networks are trained by applying back-propagation.

\subsection{Related work}
\label{sec:related-papers}


%GAN Training Improvements
Mode collapse and vanishing gradients are the most frequent pathologies regarding GAN training convergence~\cite{arjovsky2017towards,arora2017gans}, leading them to regularly get inconsistent results. 
Prior studies aimed at mitigating degenerate GAN dynamics by 
proposing new generator's or discriminator's objectives (loss functions)~\cite{arjovsky2017wasserstein,mao2017least,nguyen2017dual,zhao2016energy}, applying heuristics, e.g., decreasing the optimizer's learning rate along the iterations~\cite{Radford2015unsupervised}, or progressively increasing the number networks' layers while augmenting the images resolution~\cite{karras2017progressive}.

%Non-Evolutionary Population based GAN Training
Employing multiple generators and/or discriminators have experimentally showed been effective against training pathologies. 
Some authors have proposed 
training a cascade of GANs~\cite{wang2016ensembles};
using boosting techniques to sequentially train and add new generators~\cite{tolstikhin2017adagan},
training in parallel multiple generators and discriminators~\cite{jiwoong2016generative}, 
training an array of discriminators specialized in a different low-dimensional projection of the data~\cite{neyshabur2017stabilizing}, 
and learning ensembles of pre-trained generators~\cite{toutouh2019}. 

%Evolutionary GAN
Different strategies from EC have been also applied to deal with GAN training. 
%
Evolutionary GAN (E-GAN) evolves a population of generators using a mutation operator that updates the networks' weights by selecting randomly among three loss functions (optimization objective)~\cite{wang2018evolutionary}. 
The individuals are adversarialy trained against a single discriminator (considered optimal), which returns a fitness value for each generator. 
The use of different loss functions overcomes the limitations of using a single one and a better adapts the population to the evolution of the discriminator. 
Multi-objective E-GAN (MO-EGAN) has been defined by reformulating E-GAN training as a multi-objective optimization problem~\cite{baioletti2020multi}. 
MO-EGAN applies the same mutation function, but uses Pareto dominance to select the best solutions in terms of diversity and quality.
The preliminary results on synthetic data showed that MO-EGAN improves E-GAN.
In turn, a genetic algorithm (GA) has been proposed to evolve the GANs' architecture as a neuroevolution approach~\cite{garciarena2018evolved}. 
Thus, a single individual represents both the generator and the discriminator in the GA. 
The crossover operator combines two parents by exchanging the discriminator and the generator between them. The mutation operator varies the network architecture and training hyperparamenters.  
The fitness is computed after training the GAN encoded by the individual.
 

%Co-Evoultionary GAN
A promising research line comprises using CEAs to train a population of generators against a population of discriminators. 
Inspired by DeepNEAT~\cite{miikkulainen2019evolving}, Coevolutionary GAN (COEGAN) combines neuroevolution with CEAs~\cite{costa2019coevolution}. 
Neuroevolution is used to evolve the main networks' parameters (but not the weights and bias). 
Then, the populations of generators and discriminators apply Comp-CEA. 
The generators are evaluated in terms of the quality of the synthesized samples, e.g., by using the Fr\'echet Inception Distance (FID)~\cite{heusel2017}. 
The discriminators' fitness is computed according to the loss function. 
COEGAN applies an \textit{all-vs-best} strategy for the competitions, selecting the \textit{k best} individuals instead just one. Even though, \textit{all-vs-all}improves the variability, the computational time critically increases.     

Among CEAs, spatial ones show great success mainly due to their capability to maintain diversity and mitigate computational cost~\cite{williams2005}. 
Thus, \Lipi locates the population of GANs (pairs of generators and discriminators) in a two-dimensional toroidal grid. 
A neighborhood is defined by the cell itself and its adjacent cells according to Von Neumman neighborhood. 
Co-evolution proceeds at each cell with sub-populations drawn from the neighborhood. 
Gradient-based learning is used for GAN training (individual mutation) and evolutionary selection and variation is used for hyperparameter learning. 
After each training iteration, the \textit{best} individual generator and discriminator are propagated to the adjacent cells in four directions (i.e., North, South, East, and West). 
Thus, the sub-populations are updated with new fit individuals moving them towards convergence while fostering diversity. Another approach, Mustangs combines \Lipi and E-GAN~\cite{toutouh2019}. Inspired by E-GAN, the mutation operator randomly selects among a set of loss functions instead of applying always the same one in order to increase variability. 
Finally, taking advantage of the spatial grid of \Lipi, a \textit{data dieting} approach has been proposed~\cite{toutouh2020_dieting}. 
The main idea is to apply random sampling with replacement over the training data to define different subsets (partitions) of data that are used
as training dataset for each cell. 
This allows to foster diversity among the cells and to reduce the training resource requirements, e.g. time and memory. 

In this study, we propose \ring, a spatial distributed GAN training that uses a ring topology instead of a 2D grid. 
The idea is to evaluate how this signal propagation and new migration policies effect the quality performance and computational requirements. 

